Talking Head Generation with Probabilistic Audio-to-Visual Diffusion Priors

In this paper, we introduce a simple and novel framework for one-shot audio-driven talking head generation. Unlike prior works that require additional driving sources for controlled synthesis in a deterministic manner, we instead probabilistically sample all the holistic lip-irrelevant facial motions (i.e. pose, expression, blink, gaze, etc.) to semantically match the input audio while still maintaining both the photo-realism of audio-lip synchronization and the overall naturalness. This is achieved by our newly proposed audio-to-visual diffusion prior trained on top of the mapping between audio and disentangled non-lip facial representations. Thanks to the probabilistic nature of the diffusion prior, one big advantage of our framework is it can synthesize diverse facial motion sequences given the same audio clip, which is quite user-friendly for many real applications. Through comprehensive evaluations on public benchmarks, we conclude that (1) our diffusion prior outperforms auto-regressive prior significantly on almost all the concerned metrics; (2) our overall system is competitive with prior works in terms of audio-lip synchronization but can effectively sample rich and natural-looking lip-irrelevant facial motions while still semantically harmonized with the audio input.

==> relatedwork-_v1.tex <==
\section{Related Works}
\label{sec:relatedworks}
\paragraph{Facial Representation Learning} The recent single modality self-supervised visual representation learning\cite{chen2020simple, chen2020big,he2020momentum,chen2020improved,caron2020unsupervised,he2022masked} has received a lot of attention thanks to its generalization across various downstream visual perception tasks. Compared with pure visual self-supervised learning, CLIP \cite{radford2021learning}, ALIGN\cite{ALIGN} and BEiT series \cite{BEITV1,Beitv2,Beitv3,VL-beit} indicated that language is perhaps more effective to serve as the supervision signal for generalized pretrained visual representations. Although the progress is remarkable, little study has been shown how those models perform on the specific domain of face. \cite{zheng2022general,bulat2021pre} reported that a face-specific pretraining is still needed and showed promising results on a few limited downstream tasks. We argue that it's very challenging (if not impossible) to offer a universal facial representation that can be beneficial to all face related tasks. The key reason is that different facial analysis tasks do not necessarily share the core representations, they could even conflict with each other. For example, the head pose representation is the core for pose estimation and 3D face reconstruction task, however, it clearly should be eliminated for the face recognition task. Inspired by such observation, we hypothesize that for face synthesis tasks including face reenactments\cite{x2face2018,thies2016face2face,DeepVideoPortraits}, their best representation is different from certain analysis tasks (i.e., face recognition). Our work validated this hypothesis and filled the gap of studying a more effective pretrained representations for reenactment oriented tasks. 

%To our best knowledge, none of the prior works aim to learn a better-pretrained representation for face synthesis tasks, i.e., facial reenactment. We argue that even though face analysis and synthesis are specific vertical domains, the best representations could vary significantly across different downstream tasks. This suggests that task-oriented pretraining is much desired. 

\paragraph{Audio-Visual Cross-modal Learning} Cross-modal representation learning is a long-standing research topic, ranging from speech enhancement\cite{gabbay2017visual}, speech source separations\cite{lee2021looking} to synchronizations\cite{chung2019perfect,kadandale2022vocalist} and other speech disentanglement \cite{Nagrani20d,evp2021,Mittal_2020_WACV}. Among them, EVP \cite{evp2021} used cross-modal supervision to disentangle speech content and emotion from the audio signal with landmark as the intermediate representation. Recently, CMC \cite{CMC2020} discussed how multi-view ``modality" can be  jointly unitized to boost the intrinsic representation through constrastive learning rather than predictive (or reconstruction) learning, it also demonstrated that the more views, the better. Hence, based on the conclusion of CMC \cite{CMC2020}, EVP \cite{evp2021} is regarded as the predictive approach. Concurrently, MMV \cite{MMV2020} introduced different modality embedding graphs for effective cross-modal representations, again through constrastive learning. More recently, HCMoCo \cite{hcmoco2022} extended similar ideas with a hierarchical strategy to learn different levels of representations for human-centric perception tasks. Although impressive results were reported, it is still unclear how it performs on face analysis tasks, not mention to on synthesis tasks. Our work also follow this direction, but go one step further and introduce an iterative order-aware cross-modal constrastive learning framework, to fully respect the specificity of each modality as well as the tailored downstream reenactment-oriented tasks.

%Similarly, EVP \cite{evp2021} uses cross-modal supervision to disentangle speech content and emotion from the audio signal with landmark as the intermediate representation. Compared with EVP, the essential difference is that we jointly use visual encoding, landmark encoding as well as audio encoding to do multistage contrastive learning to learn more generalized visual and audio representations. Nevertheless, little attention has been paid to reenactment-oriented tasks powered by cross-modal visual-audio representation learning. 

\paragraph{Face Reenactment \& Talking Head Generation} Face Reenactment is designed to transfer part or full facial motion from a driving source to reenact the face in the target video while preserving its identity and the background. It can be further divided into two categories depending on whether the driving source is from video \cite{hong2022depth,hsu2022dual,bounareli2022finding,thies2016face2face,DeepVideoPortraits,x2face2018,Zakharov_2019_ICCV,huang2020learning,Zeng2020,Burkov_2020_CVPR} or audio \cite{IJCV2019RealisticGAN,thies2020nvp,APB2Face2020,evp2021}. Among them, audio-driven face reenactment generally aims to edit the mouth regions of the target video in order to match the input audio while leaving other facial attributes mostly unchanged, i.e., pose. EVP \cite{evp2021} tries to infer the non-rigid facial expression in addition to lip motion from audio input. A closely related line of work is the audio-driven talking-head generations \cite{wav2lip,zhou2020makelttalk,zhang2021facial,alghamdi2022talking} where only one target reference face is given, hence, other face attributes including pose, expression, eye blinks and gaze have to be either explicitly given \cite{zhou2021pose,Liang_2022_CVPR} or statistically inferred \cite{zhou2020makelttalk,min2022styletalker,zhang2021facial,lu2021live,alghamdi2022talking,thies2020nvp}. Specifically, Lu \etal \cite{lu2021live} employed an auto-regressive model while Min \etal \cite{min2022styletalker} leveraged normalized flow prior to predicting a natural-looking head pose sequence from the input audio, both showed impressive results. Different from all those prior works which target solving specific downstream tasks individually, we propose to pretrain both visual and audio representations holistically in one unified framework to benefit all the related face reenactment and talking head generation tasks. 
\paragraph{Diffusion Generative Models}
Recently, diffusion models \cite{sohl2015deep, ho2020denoising, song2020denoising} have witnessed great progress in image generation\cite{dhariwal2021diffusion, nichol2021glide, ramesh2022hierarchical, rombach2022high}, audio generation\cite{kong2020diffwave}, video generation\cite{singer2022make} as well as motion generation\cite{tevet2022human}. It's a class of generative model, based on the stochastic diffusion process. Specifically, DDPM\cite{ho2020denoising} utilized the diffusion model for unconditional image generation. GLIDE\cite{nichol2021glide} explored  CLIP\cite{radford2021learning} guidance and classifier-free
guidance for text-conditional image synthesis. DALLE2\cite{ramesh2022hierarchical} proposed to learn a diffusion prior to map text encodings to the image encoding space of CLIP, demonstrating better diversity than a autoregressive prior. MDM\cite{tevet2022human} also utilized a diffusion prior to learn one-to-many dynamics in text-to-motion generation and action-to-motion tasks. Inspired by these works, we propose to learn a diffusion prior in talking head generation, to model the one-to-many dynamics (i.e., dynamic pose and expression) while talking. To the best of our knowledge, none of the existing works apply diffusion models to address one-to-many problems in  audio-to-visual scenario. 
% \paragraph{Face Swap}
% \paragraph{Talking Head Generation}
% \usepackage{graphicx} % 需使用包

